Dissipation in mesoscale superfluids

We investigate the maximum speed at which a driven superfluid can flow through a narrow constriction with a size on the order of the healing length. Considering dissipation via the thermal nucleation of quantized vortices, we calculate the critical velocity for superfluid $^4$He and ultracold atomtronic circuits, identify fundamental length and velocity scales, and are thus able to present results obtained in widely different temperature and density ranges in a universal framework. For ultra-narrow channels we predict a drastic reduction in the critical velocity as the energy barrier for flow reducing thermally activated phase slip fluctuations is suppressed.

==> main_refs.tex <==
\begin{thebibliography}{69}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Anderson}(1966)}]{anderson}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Anderson}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Considerations on the Flow of Superfluid Helium}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Rev. Mod. Phys.}\ }\textbf
  {\bibinfo {volume} {38}},\ \bibinfo {pages} {298} (\bibinfo {year}
  {1966})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Varoquaux}(2015)}]{varoquauxrmp}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Eric}\ \bibnamefont
  {Varoquaux}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Anderson{\textquoteright}s considerations on the flow of superfluid helium:
  Some offshoots}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {87}},\ \bibinfo {pages} {803}
  (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chien}\ \emph {et~al.}(2015)\citenamefont {Chien},
  \citenamefont {Peotta},\ and\ \citenamefont {Di~Ventra}}]{chien}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Chih-Chun}\
  \bibnamefont {Chien}}, \bibinfo {author} {\bibfnamefont {Sebastiano}\
  \bibnamefont {Peotta}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Massimiliano}\ \bibnamefont {Di~Ventra}},\ }\bibfield  {title} {\enquote
  {\bibinfo {title} {{Quantum transport in ultracold atoms}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature Phys.}\ }\textbf {\bibinfo
  {volume} {11}},\ \bibinfo {pages} {998} (\bibinfo {year} {2015})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sato}\ and\ \citenamefont {Packard}(2012)}]{sato}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Yuki}\ \bibnamefont
  {Sato}}\ and\ \bibinfo {author} {\bibfnamefont {Richard}\ \bibnamefont
  {Packard}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Superfluid
  helium interferometers}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Today}\ }\textbf {\bibinfo {volume} {65}},\ \bibinfo {pages}
  {31} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schumm}\ \emph {et~al.}(2005)\citenamefont {Schumm},
  \citenamefont {Hofferberth}, \citenamefont {Andersson}, \citenamefont
  {Wildermuth}, \citenamefont {Groth}, \citenamefont {Bar-Joseph},
  \citenamefont {Schmiedmayer},\ and\ \citenamefont {Kruger}}]{Schumm+05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Schumm}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Hofferberth}},
  \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Andersson}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Wildermuth}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Groth}}, \bibinfo {author} {\bibfnamefont
  {I.}~\bibnamefont {Bar-Joseph}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Schmiedmayer}}, \ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Kruger}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {Matter-wave interferometry in a double well on an atom chip},}\ }\href
  {http://dx.doi.org/10.1038/nphys125} {\bibfield  {journal} {\bibinfo
  {journal} {Nat Phys}\ }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages}
  {57--62} (\bibinfo {year} {2005})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chiow}\ \emph {et~al.}(2011)\citenamefont {Chiow},
  \citenamefont {Kovachy}, \citenamefont {Chien},\ and\ \citenamefont
  {Kasevich}}]{Chiow+11}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Sheng-wey}\
  \bibnamefont {Chiow}}, \bibinfo {author} {\bibfnamefont {Tim}\ \bibnamefont
  {Kovachy}}, \bibinfo {author} {\bibfnamefont {Hui-Chun}\ \bibnamefont
  {Chien}}, \ and\ \bibinfo {author} {\bibfnamefont {Mark~A.}\ \bibnamefont
  {Kasevich}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {$102\ensuremath{\hbar}k$ large area atom interferometers},}\ }\href
  {\doibase 10.1103/PhysRevLett.107.130403} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {107}},\ \bibinfo
  {pages} {130403} (\bibinfo {year} {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hoskinson}\ \emph
  {et~al.}(2005{\natexlab{a}})\citenamefont {Hoskinson}, \citenamefont
  {Packard},\ and\ \citenamefont {Haard}}]{Hoskinson:2005km}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Hoskinson}}, \bibinfo {author} {\bibfnamefont {R.~E.}\ \bibnamefont
  {Packard}}, \ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Haard}, \bibfnamefont {Thomas}},\ }\bibfield  {title} {\enquote {\bibinfo
  {title} {{Oscillatory motion: Quantum whistling in superfluid helium-4}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf
  {\bibinfo {volume} {433}},\ \bibinfo {pages} {376} (\bibinfo {year}
  {2005}{\natexlab{a}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hoskinson}\ \emph
  {et~al.}(2005{\natexlab{b}})\citenamefont {Hoskinson}, \citenamefont {Sato},
  \citenamefont {Hahn},\ and\ \citenamefont {Packard}}]{hoskinson}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Hoskinson}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Sato}},
  \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Hahn}}, \ and\ \bibinfo
  {author} {\bibfnamefont {R.~E.}\ \bibnamefont {Packard}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Transition from phase slips to the
  Josephson effect in a superfluid 4He weak~link}},}\ }\href@noop {} {\bibfield
   {journal} {\bibinfo  {journal} {Nature Phys.}\ }\textbf {\bibinfo {volume}
  {2}},\ \bibinfo {pages} {23} (\bibinfo {year}
  {2005}{\natexlab{b}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cheng}\ \emph {et~al.}(2015)\citenamefont {Cheng},
  \citenamefont {Beamish}, \citenamefont {Fefferman}, \citenamefont {Souris},
  \citenamefont {Balibar},\ and\ \citenamefont {Dauvois}}]{Cheng:2015yh}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Zhi~Gang}\
  \bibnamefont {Cheng}}, \bibinfo {author} {\bibfnamefont {John}\ \bibnamefont
  {Beamish}}, \bibinfo {author} {\bibfnamefont {Andrew~D.}\ \bibnamefont
  {Fefferman}}, \bibinfo {author} {\bibfnamefont {Fabien}\ \bibnamefont
  {Souris}}, \bibinfo {author} {\bibfnamefont {S\'ebastien}\ \bibnamefont
  {Balibar}}, \ and\ \bibinfo {author} {\bibfnamefont {Vincent}\ \bibnamefont
  {Dauvois}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {Helium mass
  flow through a solid-superfluid-solid junction},}\ }\href {\doibase
  10.1103/PhysRevLett.114.165301} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {114}},\ \bibinfo {pages}
  {165301} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cheng}\ and\ \citenamefont
  {Beamish}(2016)}]{beamish:2016ay}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Zhi~Gang}\
  \bibnamefont {Cheng}}\ and\ \bibinfo {author} {\bibfnamefont {John}\
  \bibnamefont {Beamish}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {Compression-driven mass flow in bulk solid $^{4}\mathrm{He}$},}\ }\href
  {\doibase 10.1103/PhysRevLett.117.025301} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {117}},\ \bibinfo
  {pages} {025301} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vekhov}\ \emph {et~al.}(2014)\citenamefont {Vekhov},
  \citenamefont {Mullin},\ and\ \citenamefont {Hallock}}]{Vekhov:2014ym}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Vekhov}}, \bibinfo {author} {\bibfnamefont {W.~J.}\ \bibnamefont {Mullin}},
  \ and\ \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont {Hallock}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {Universal temperature
  dependence, flux extinction, and the role of $^{3}\mathrm{He}$ impurities in
  superfluid mass transport through solid $^{4}\mathrm{He}$},}\ }\href
  {\doibase 10.1103/PhysRevLett.113.035302} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {113}},\ \bibinfo
  {pages} {035302} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vekhov}\ and\ \citenamefont
  {Hallock}(2012)}]{Vekhov:2012mf}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Vekhov}}\ and\ \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont
  {Hallock}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Mass Flux
  Characteristics in Solid $^4$He for $T > 100$~mK: Evidence for Bosonic
  Luttinger-Liquid Behavior}},}\ }\href {\doibase
  10.1103/PhysRevLett.109.045303} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {109}},\ \bibinfo {pages}
  {045303} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ray}\ and\ \citenamefont
  {Hallock}(2010)}]{Ray:2010mf}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~W.}\ \bibnamefont
  {Ray}}\ and\ \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont
  {Hallock}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {Mass flux and
  solid growth in solid $^{4}\mathrm{He}$ for 60--700 mk},}\ }\href {\doibase
  10.1103/PhysRevLett.105.145301} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {105}},\ \bibinfo {pages}
  {145301} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ray}\ and\ \citenamefont
  {Hallock}(2008)}]{Ray:2008ou}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~W.}\ \bibnamefont
  {Ray}}\ and\ \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont
  {Hallock}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {Observation of
  unusual mass transport in solid hcp $^{4}\mathrm{He}$},}\ }\href {\doibase
  10.1103/PhysRevLett.100.235301} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo {pages}
  {235301} (\bibinfo {year} {2008})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Boninsegni}\ \emph {et~al.}(2007)\citenamefont
  {Boninsegni}, \citenamefont {Kuklov}, \citenamefont {Pollet}, \citenamefont
  {Prokof'ev}, \citenamefont {Svistunov},\ and\ \citenamefont
  {Troyer}}]{Boninsegni:2007ll}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Boninsegni}}, \bibinfo {author} {\bibfnamefont {A.~B.}\ \bibnamefont
  {Kuklov}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Pollet}},
  \bibinfo {author} {\bibfnamefont {N.~V.}\ \bibnamefont {Prokof'ev}}, \bibinfo
  {author} {\bibfnamefont {B.~V.}\ \bibnamefont {Svistunov}}, \ and\ \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Troyer}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {Luttinger liquid in the core of a screw
  dislocation in helium-4},}\ }\href {\doibase 10.1103/PhysRevLett.99.035301}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {99}},\ \bibinfo {pages} {035301} (\bibinfo {year}
  {2007})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Savard}\ \emph {et~al.}(2011)\citenamefont {Savard},
  \citenamefont {Dauphinais},\ and\ \citenamefont {Gervais}}]{Savard:2011hs}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Savard}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Dauphinais}},
  \ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Gervais}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {Hydrodynamics of superfluid
  helium in a single nanohole},}\ }\href {\doibase
  10.1103/PhysRevLett.107.254501} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {107}},\ \bibinfo {pages}
  {254501} (\bibinfo {year} {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Savard}\ \emph {et~al.}(2009)\citenamefont {Savard},
  \citenamefont {Tremblay-Darveau},\ and\ \citenamefont
  {Gervais}}]{Savard:2009fc}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Savard}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Tremblay-Darveau}}, \ and\ \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Gervais}},\ }\bibfield  {title} {\enquote {\bibinfo
  {title} {Flow conductance of a single nanohole},}\ }\href {\doibase
  10.1103/PhysRevLett.103.104502} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {103}},\ \bibinfo {pages}
  {104502} (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Duc}\ \emph {et~al.}(2015)\citenamefont {Duc},
  \citenamefont {Savard}, \citenamefont {Petrescu}, \citenamefont {Rosenow},
  \citenamefont {Del~Maestro},\ and\ \citenamefont {Gervais}}]{duc}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Pierre-Francois}\
  \bibnamefont {Duc}}, \bibinfo {author} {\bibfnamefont {Michel}\ \bibnamefont
  {Savard}}, \bibinfo {author} {\bibfnamefont {Matei}\ \bibnamefont
  {Petrescu}}, \bibinfo {author} {\bibfnamefont {Bernd}\ \bibnamefont
  {Rosenow}}, \bibinfo {author} {\bibfnamefont {Adrian}\ \bibnamefont
  {Del~Maestro}}, \ and\ \bibinfo {author} {\bibfnamefont {Guillaume}\
  \bibnamefont {Gervais}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Critical flow and dissipation in a quasi-one-dimensional superfluid}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Science Adv.}\
  }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages} {e1400222} (\bibinfo
  {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Velasco}\ \emph {et~al.}(2012)\citenamefont
  {Velasco}, \citenamefont {Friedman}, \citenamefont {Pevarnik}, \citenamefont
  {Siwy},\ and\ \citenamefont {Taborek}}]{Velasco:2012de}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~E.}\ \bibnamefont
  {Velasco}}, \bibinfo {author} {\bibfnamefont {S.~G.}\ \bibnamefont
  {Friedman}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Pevarnik}},
  \bibinfo {author} {\bibfnamefont {Z.~S.}\ \bibnamefont {Siwy}}, \ and\
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Taborek}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Pressure-driven flow through a single
  nanopore}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. E}\ }\textbf {\bibinfo {volume} {86}},\ \bibinfo {pages} {025302}
  (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Velasco}\ \emph {et~al.}(2014)\citenamefont
  {Velasco}, \citenamefont {Yang}, \citenamefont {Siwy}, \citenamefont
  {Toimil-Molares},\ and\ \citenamefont {Taborek}}]{velasco}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~E.}\ \bibnamefont
  {Velasco}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Yang}},
  \bibinfo {author} {\bibfnamefont {Z.~S.}\ \bibnamefont {Siwy}}, \bibinfo
  {author} {\bibfnamefont {M.~E.}\ \bibnamefont {Toimil-Molares}}, \ and\
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Taborek}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Flow and evaporation in single
  micrometer and nanometer scale pipes}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Applied Physics Lett.}\ }\textbf {\bibinfo
  {volume} {105}},\ \bibinfo {pages} {033101} (\bibinfo {year}
  {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Botimer}\ and\ \citenamefont
  {Taborek}(2016)}]{Botimer:2016pd}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Jeffrey}\ \bibnamefont
  {Botimer}}\ and\ \bibinfo {author} {\bibfnamefont {Peter}\ \bibnamefont
  {Taborek}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {Pressure driven
  flow of superfluid $^{4}\mathrm{He}$ through a nanopipe},}\ }\href {\doibase
  10.1103/PhysRevFluids.1.054102} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Fluids}\ }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages}
  {054102} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fil}\ and\ \citenamefont
  {Shevchenko}(2009)}]{Fil:2009bpa}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~V.}\ \bibnamefont
  {Fil}}\ and\ \bibinfo {author} {\bibfnamefont {S.~I.}\ \bibnamefont
  {Shevchenko}},\ }\bibfield  {title} {{\selectlanguage {English}\enquote
  {\bibinfo {title} {{Relaxation of superflow in a network: Application to the
  dislocation model of supersolidity of helium crystals}},}\ }}\href {\doibase
  10.1103/PhysRevB.80.100501} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {80}},\ \bibinfo {pages} {100501}
  (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Del~Maestro}\ \emph {et~al.}(2011)\citenamefont
  {Del~Maestro}, \citenamefont {Boninsegni},\ and\ \citenamefont
  {Affleck}}]{DelMaestro:2011ll}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Adrian}\ \bibnamefont
  {Del~Maestro}}, \bibinfo {author} {\bibfnamefont {Massimo}\ \bibnamefont
  {Boninsegni}}, \ and\ \bibinfo {author} {\bibfnamefont {Ian}\ \bibnamefont
  {Affleck}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {$^{4}\mathrm{He}$ luttinger liquid in nanopores},}\ }\href {\doibase
  10.1103/PhysRevLett.106.105303} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {106}},\ \bibinfo {pages}
  {105303} (\bibinfo {year} {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pollet}\ and\ \citenamefont
  {Kuklov}(2014)}]{Pollet:2014tq}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Lode}\ \bibnamefont
  {Pollet}}\ and\ \bibinfo {author} {\bibfnamefont {Anatoly~B.}\ \bibnamefont
  {Kuklov}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {Topological
  quantum phases of $^{4}\mathrm{He}$ confined to nanoporous materials},}\
  }\href {\doibase 10.1103/PhysRevLett.113.045301} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {113}},\
  \bibinfo {pages} {045301} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Raman}\ \emph {et~al.}(1999)\citenamefont {Raman},
  \citenamefont {K{\"o}hl}, \citenamefont {Onofrio}, \citenamefont {Durfee},
  \citenamefont {Kuklewicz}, \citenamefont {Hadzibabic},\ and\ \citenamefont
  {Ketterle}}]{raman}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Raman}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {K{\"o}hl}},
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Onofrio}}, \bibinfo
  {author} {\bibfnamefont {D.~S.}\ \bibnamefont {Durfee}}, \bibinfo {author}
  {\bibfnamefont {C.~E.}\ \bibnamefont {Kuklewicz}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Hadzibabic}}, \ and\ \bibinfo {author}
  {\bibfnamefont {W.}~\bibnamefont {Ketterle}},\ }\bibfield  {title} {\enquote
  {\bibinfo {title} {{Evidence for a Critical Velocity in a Bose-Einstein
  Condensed Gas}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {83}},\ \bibinfo {pages}
  {2502} (\bibinfo {year} {1999})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Watanabe}\ \emph {et~al.}(2009)\citenamefont
  {Watanabe}, \citenamefont {Dalfovo}, \citenamefont {Piazza}, \citenamefont
  {Pitaevskii},\ and\ \citenamefont {Stringari}}]{watanabe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Gentaro}\ \bibnamefont
  {Watanabe}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Dalfovo}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Piazza}}, \bibinfo
  {author} {\bibfnamefont {L.~P.}\ \bibnamefont {Pitaevskii}}, \ and\ \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Stringari}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Critical velocity of superfluid flow through
  single-barrier and periodic potentials}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume}
  {80}},\ \bibinfo {pages} {053602} (\bibinfo {year} {2009})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Neely}\ \emph {et~al.}(2010)\citenamefont {Neely},
  \citenamefont {Samson}, \citenamefont {Bradley}, \citenamefont {Davis},\ and\
  \citenamefont {Anderson}}]{neely}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.~W.}\ \bibnamefont
  {Neely}}, \bibinfo {author} {\bibfnamefont {E.~C.}\ \bibnamefont {Samson}},
  \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont {Bradley}}, \bibinfo
  {author} {\bibfnamefont {M.~J.}\ \bibnamefont {Davis}}, \ and\ \bibinfo
  {author} {\bibfnamefont {B.~P.}\ \bibnamefont {Anderson}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Observation of Vortex Dipoles in an
  Oblate Bose-Einstein Condensate}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {104}},\
  \bibinfo {pages} {160401} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ramanathan}\ \emph {et~al.}(2011)\citenamefont
  {Ramanathan}, \citenamefont {Wright}, \citenamefont {Muniz}, \citenamefont
  {Zelan}, \citenamefont {Hill}, \citenamefont {Lobb}, \citenamefont
  {Helmerson}, \citenamefont {Phillips},\ and\ \citenamefont
  {Campbell}}]{ramanathan}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Ramanathan}}, \bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont
  {Wright}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Muniz}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Zelan}}, \bibinfo
  {author} {\bibfnamefont {W.~T.}\ \bibnamefont {Hill}}, \bibinfo {author}
  {\bibfnamefont {C.~J.}\ \bibnamefont {Lobb}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Helmerson}}, \bibinfo {author}
  {\bibfnamefont {W.~D.}\ \bibnamefont {Phillips}}, \ and\ \bibinfo {author}
  {\bibfnamefont {G.~K.}\ \bibnamefont {Campbell}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Superflow in a Toroidal Bose-Einstein
  Condensate: An Atom Circuit with a Tunable Weak Link}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {106}},\ \bibinfo {pages} {130401} (\bibinfo {year}
  {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lee}\ \emph {et~al.}(2013)\citenamefont {Lee},
  \citenamefont {McIlvain}, \citenamefont {Lobb},\ and\ \citenamefont
  {T.}}]{lee}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Jeffrey~G.}\
  \bibnamefont {Lee}}, \bibinfo {author} {\bibfnamefont {Brian~J.}\
  \bibnamefont {McIlvain}}, \bibinfo {author} {\bibfnamefont {C.~J.}\
  \bibnamefont {Lobb}}, \ and\ \bibinfo {author} {\bibfnamefont {Hill~W.}\
  \bibnamefont {T.}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Analogs of Basic Electronic Circuit Elements in a Free-Space Atom Chip}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Sci. Rep.}\
  }\textbf {\bibinfo {volume} {3}},\ \bibinfo {pages} {1034} (\bibinfo {year}
  {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wright}\ \emph
  {et~al.}(2013{\natexlab{a}})\citenamefont {Wright}, \citenamefont
  {Blakestad}, \citenamefont {Lobb}, \citenamefont {Phillips},\ and\
  \citenamefont {Campbell}}]{wright}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont
  {Wright}}, \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont
  {Blakestad}}, \bibinfo {author} {\bibfnamefont {C.~J.}\ \bibnamefont {Lobb}},
  \bibinfo {author} {\bibfnamefont {W.~D.}\ \bibnamefont {Phillips}}, \ and\
  \bibinfo {author} {\bibfnamefont {G.~K.}\ \bibnamefont {Campbell}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {{Driving Phase Slips in a
  Superfluid Atom Circuit with a Rotating Weak Link}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {110}},\ \bibinfo {pages} {025302} (\bibinfo {year}
  {2013}{\natexlab{a}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Murray}\ \emph {et~al.}(2013)\citenamefont {Murray},
  \citenamefont {Krygier}, \citenamefont {Edwards}, \citenamefont {Wright},
  \citenamefont {Campbell},\ and\ \citenamefont {Clark}}]{Murray:2013br}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Noel}\ \bibnamefont
  {Murray}}, \bibinfo {author} {\bibfnamefont {Michael}\ \bibnamefont
  {Krygier}}, \bibinfo {author} {\bibfnamefont {Mark}\ \bibnamefont {Edwards}},
  \bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont {Wright}}, \bibinfo
  {author} {\bibfnamefont {G.~K.}\ \bibnamefont {Campbell}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Charles~W.}\ \bibnamefont {Clark}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Probing the circulation of ring-shaped
  Bose-Einstein condensates}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
   {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {88}},\ \bibinfo
  {pages} {053615} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wright}\ \emph
  {et~al.}(2013{\natexlab{b}})\citenamefont {Wright}, \citenamefont
  {Blakestad}, \citenamefont {Lobb}, \citenamefont {Phillips},\ and\
  \citenamefont {Campbell}}]{Wright:2013bg}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont
  {Wright}}, \bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont
  {Blakestad}}, \bibinfo {author} {\bibfnamefont {C.~J.}\ \bibnamefont {Lobb}},
  \bibinfo {author} {\bibfnamefont {W.~D.}\ \bibnamefont {Phillips}}, \ and\
  \bibinfo {author} {\bibfnamefont {G.~K.}\ \bibnamefont {Campbell}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {{Threshold for creating
  excitations in a stirred superfluid ring}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume}
  {88}},\ \bibinfo {pages} {063633} (\bibinfo {year}
  {2013}{\natexlab{b}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Eckel}\ \emph {et~al.}(2014)\citenamefont {Eckel},
  \citenamefont {Lee}, \citenamefont {Jendrzejewski}, \citenamefont {Murray},
  \citenamefont {Clark}, \citenamefont {Lobb}, \citenamefont {Phillips},
  \citenamefont {Edwards},\ and\ \citenamefont {Campbell}}]{eckel}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Stephen}\ \bibnamefont
  {Eckel}}, \bibinfo {author} {\bibfnamefont {Jeffrey~G}\ \bibnamefont {Lee}},
  \bibinfo {author} {\bibfnamefont {Fred}\ \bibnamefont {Jendrzejewski}},
  \bibinfo {author} {\bibfnamefont {Noel}\ \bibnamefont {Murray}}, \bibinfo
  {author} {\bibfnamefont {Charles~W}\ \bibnamefont {Clark}}, \bibinfo {author}
  {\bibfnamefont {Christopher~J}\ \bibnamefont {Lobb}}, \bibinfo {author}
  {\bibfnamefont {William~D}\ \bibnamefont {Phillips}}, \bibinfo {author}
  {\bibfnamefont {Mark}\ \bibnamefont {Edwards}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Gretchen~K}\ \bibnamefont {Campbell}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Hysteresis in a quantized superfluid
  `atomtronic' circuit}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Nature}\ }\textbf {\bibinfo {volume} {506}},\ \bibinfo {pages}
  {200} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jendrzejewski}\ \emph {et~al.}(2014)\citenamefont
  {Jendrzejewski}, \citenamefont {Eckel}, \citenamefont {Murray}, \citenamefont
  {Lanier}, \citenamefont {Edwards}, \citenamefont {Lobb},\ and\ \citenamefont
  {Campbell}}]{Jendrzejewski:2014dy}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F}~\bibnamefont
  {Jendrzejewski}}, \bibinfo {author} {\bibfnamefont {S}~\bibnamefont {Eckel}},
  \bibinfo {author} {\bibfnamefont {N}~\bibnamefont {Murray}}, \bibinfo
  {author} {\bibfnamefont {C}~\bibnamefont {Lanier}}, \bibinfo {author}
  {\bibfnamefont {M}~\bibnamefont {Edwards}}, \bibinfo {author} {\bibfnamefont
  {C~J}\ \bibnamefont {Lobb}}, \ and\ \bibinfo {author} {\bibfnamefont {G~K}\
  \bibnamefont {Campbell}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Resistive Flow in a Weakly Interacting Bose-Einstein Condensate}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\
  }\textbf {\bibinfo {volume} {113}},\ \bibinfo {pages} {045305} (\bibinfo
  {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mathey}\ \emph {et~al.}(2014)\citenamefont {Mathey},
  \citenamefont {Clark},\ and\ \citenamefont {Mathey}}]{mathey}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Amy~C.}\ \bibnamefont
  {Mathey}}, \bibinfo {author} {\bibfnamefont {Charles~W.}\ \bibnamefont
  {Clark}}, \ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Mathey}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Decay of a
  superfluid current of ultracold atoms in a toroidal trap}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo
  {volume} {90}},\ \bibinfo {pages} {023604} (\bibinfo {year}
  {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Weimer}\ \emph {et~al.}(2015)\citenamefont {Weimer},
  \citenamefont {Morgener}, \citenamefont {Singh}, \citenamefont {Siegl},
  \citenamefont {Hueck}, \citenamefont {Luick}, \citenamefont {Mathey},\ and\
  \citenamefont {Moritz}}]{weimer}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Wolf}\ \bibnamefont
  {Weimer}}, \bibinfo {author} {\bibfnamefont {Kai}\ \bibnamefont {Morgener}},
  \bibinfo {author} {\bibfnamefont {Vijay~Pal}\ \bibnamefont {Singh}}, \bibinfo
  {author} {\bibfnamefont {Jonas}\ \bibnamefont {Siegl}}, \bibinfo {author}
  {\bibfnamefont {Klaus}\ \bibnamefont {Hueck}}, \bibinfo {author}
  {\bibfnamefont {Niclas}\ \bibnamefont {Luick}}, \bibinfo {author}
  {\bibfnamefont {Ludwig}\ \bibnamefont {Mathey}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Henning}\ \bibnamefont {Moritz}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Critical Velocity in the BEC-BCS Crossover}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\
  }\textbf {\bibinfo {volume} {114}},\ \bibinfo {pages} {095301} (\bibinfo
  {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Husmann}\ \emph {et~al.}(2015)\citenamefont
  {Husmann}, \citenamefont {Uchino}, \citenamefont {Krinner}, \citenamefont
  {Lebrat}, \citenamefont {Giamarchi}, \citenamefont {Esslinger},\ and\
  \citenamefont {Brantut}}]{husmann}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Dominik}\ \bibnamefont
  {Husmann}}, \bibinfo {author} {\bibfnamefont {Shun}\ \bibnamefont {Uchino}},
  \bibinfo {author} {\bibfnamefont {Sebastian}\ \bibnamefont {Krinner}},
  \bibinfo {author} {\bibfnamefont {Martin}\ \bibnamefont {Lebrat}}, \bibinfo
  {author} {\bibfnamefont {Thierry}\ \bibnamefont {Giamarchi}}, \bibinfo
  {author} {\bibfnamefont {Tilman}\ \bibnamefont {Esslinger}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Jean-Philippe}\ \bibnamefont {Brantut}},\ }\bibfield
   {title} {\enquote {\bibinfo {title} {{Connecting strongly correlated
  superfluids by a quantum point contact}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo {volume}
  {350}},\ \bibinfo {pages} {1498} (\bibinfo {year} {2015})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Singh}\ \emph {et~al.}(2016)\citenamefont {Singh},
  \citenamefont {Weimer}, \citenamefont {Morgener}, \citenamefont {Siegl},
  \citenamefont {Hueck}, \citenamefont {Luick}, \citenamefont {Moritz},\ and\
  \citenamefont {Mathey}}]{singh}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Vijay~Pal}\
  \bibnamefont {Singh}}, \bibinfo {author} {\bibfnamefont {Wolf}\ \bibnamefont
  {Weimer}}, \bibinfo {author} {\bibfnamefont {Kai}\ \bibnamefont {Morgener}},
  \bibinfo {author} {\bibfnamefont {Jonas}\ \bibnamefont {Siegl}}, \bibinfo
  {author} {\bibfnamefont {Klaus}\ \bibnamefont {Hueck}}, \bibinfo {author}
  {\bibfnamefont {Niclas}\ \bibnamefont {Luick}}, \bibinfo {author}
  {\bibfnamefont {Henning}\ \bibnamefont {Moritz}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Ludwig}\ \bibnamefont {Mathey}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Probing superfluidity of Bose-Einstein
  condensates via laser stirring}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {93}},\
  \bibinfo {pages} {023634} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Li}\ \emph {et~al.}(2016)\citenamefont {Li},
  \citenamefont {Eckel}, \citenamefont {Eller}, \citenamefont {Warren},
  \citenamefont {Clark},\ and\ \citenamefont {Edwards}}]{Li:2016ux}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Aijun}\ \bibnamefont
  {Li}}, \bibinfo {author} {\bibfnamefont {Stephen}\ \bibnamefont {Eckel}},
  \bibinfo {author} {\bibfnamefont {Benjamin}\ \bibnamefont {Eller}}, \bibinfo
  {author} {\bibfnamefont {Kayla~E}\ \bibnamefont {Warren}}, \bibinfo {author}
  {\bibfnamefont {Charles~W}\ \bibnamefont {Clark}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Mark}\ \bibnamefont {Edwards}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Superfluid transport dynamics in a capacitive
  atomtronic circuit}},}\ }\href@noop {} {\  (\bibinfo {year} {2016})},\
  \Eprint {http://arxiv.org/abs/1606.02758} {1606.02758} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Landau}(1941)}]{landau}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Landau}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Theory of the
  Superfluidity of Helium II}},}\ }\href {\doibase 10.1103/PhysRev.60.356}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev.}\ }\textbf {\bibinfo
  {volume} {60}},\ \bibinfo {pages} {356--358} (\bibinfo {year}
  {1941})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Iordanskii}(1965)}]{iordanskii}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~V.}\ \bibnamefont
  {Iordanskii}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Vortex ring
  formation in a superfluid}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
   {journal} {Sov. Phys. JETP}\ }\textbf {\bibinfo {volume} {21}},\ \bibinfo
  {pages} {467} (\bibinfo {year} {1965})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Feynman}(1955)}]{feynman}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~P.}\ \bibnamefont
  {Feynman}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Application of
  quantum mechanics to liquid helium}},}\ }in\ \href@noop {} {\emph {\bibinfo
  {booktitle} {Prog. in Low Temp. Phys.}}},\ Vol.~\bibinfo {volume} {1}\
  (\bibinfo {address} {Amsterdam},\ \bibinfo {year} {1955})\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Langer}\ and\ \citenamefont {Fisher}(1967)}]{langer}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Langer}}\ and\ \bibinfo {author} {\bibfnamefont {Michael}\ \bibnamefont
  {Fisher}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Intrinsic
  Critical Velocity of a Superfluid}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {19}},\
  \bibinfo {pages} {560} (\bibinfo {year} {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Volovik}(1972)}]{volovik}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.~E.}\ \bibnamefont
  {Volovik}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Quantum-mechanical formation of vortices in a superfluid liquid}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Sov. Phys. JETP}\
  }\textbf {\bibinfo {volume} {58}},\ \bibinfo {pages} {458} (\bibinfo {year}
  {1972})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Harrison}\ and\ \citenamefont
  {Mendelssohn}(1974)}]{harrison}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~J.}\ \bibnamefont
  {Harrison}}\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Mendelssohn}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Superfluid
  4He Velocities in Narrow Channels between 1.8 and 0.3 K}},}\ }in\ \href@noop
  {} {\emph {\bibinfo {booktitle} {Low Temperature Physics}}},\ \bibinfo
  {editor} {edited by\ \bibinfo {editor} {\bibfnamefont {T~D}\ \bibnamefont
  {Timmerhaus}}}\ (\bibinfo  {publisher} {Springer},\ \bibinfo {address} {New
  York},\ \bibinfo {year} {1974})\ p.\ \bibinfo {pages} {298}\BibitemShut
  {NoStop}%
\bibitem [{sup()}]{supplemental}%
  \BibitemOpen
  \href@noop {} {}\bibinfo {note} {{See Supplemental Material for details on
  potential flow, vortex energies, experimental comparisons, and the critical
  velocity in the $a/\xi \gg 1$ and $a/\xi \approx 1$ limits.}}\BibitemShut
  {Stop}%
\bibitem [{\citenamefont {Pitaevskii}(1961)}]{Pi61}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~P.}\ \bibnamefont
  {Pitaevskii}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Vortex
  lines in an imperfect Bose gas}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Sov. Phys. JETP}\ }\textbf {\bibinfo {volume} {13}},\
  \bibinfo {pages} {451} (\bibinfo {year} {1961})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Roberts}\ and\ \citenamefont {Grant}(1971)}]{RoGr71}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.~H.}\ \bibnamefont
  {Roberts}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Grant}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Motions in a
  Bose condensate. I. The structure of the large circular vortex}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. A: Gen.
  Phys.}\ }\textbf {\bibinfo {volume} {4}},\ \bibinfo {pages} {55} (\bibinfo
  {year} {1971})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Winiecki}\ \emph {et~al.}(1999)\citenamefont
  {Winiecki}, \citenamefont {McCann},\ and\ \citenamefont {Adams}}]{Wi99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Winiecki}}, \bibinfo {author} {\bibfnamefont {J.~F.}\ \bibnamefont
  {McCann}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~S.}\ \bibnamefont
  {Adams}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Vortex
  structures in dilute quantum fluids}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Europhys. Lett.}\ }\textbf {\bibinfo {volume} {48}},\
  \bibinfo {pages} {475} (\bibinfo {year} {1999})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ortiz}\ and\ \citenamefont
  {Ceperley}(1995)}]{OrCe95}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Gerardo}\ \bibnamefont
  {Ortiz}}\ and\ \bibinfo {author} {\bibfnamefont {David~M}\ \bibnamefont
  {Ceperley}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Core
  Structure of a Vortex in Superfluid He4}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {4642} (\bibinfo {year}
  {1995})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Galli}\ \emph {et~al.}(2014)\citenamefont {Galli},
  \citenamefont {Reatto},\ and\ \citenamefont {Rossi}}]{GaReRo14}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~E.}\ \bibnamefont
  {Galli}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Reatto}}, \
  and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Rossi}},\ }\bibfield
   {title} {\enquote {\bibinfo {title} {{Quantum Monte Carlo study of a vortex
  in superfluid 4He and search for a vortex state in the solid}},}\ }\href@noop
  {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf
  {\bibinfo {volume} {89}},\ \bibinfo {pages} {224516} (\bibinfo {year}
  {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Josephson}(1966)}]{josephson}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.~D.}\ \bibnamefont
  {Josephson}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Relation
  between the superfluid density and order parameter for superfluid He near
  Tc}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Lett.}\ }\textbf {\bibinfo {volume} {21}},\ \bibinfo {pages} {608} (\bibinfo
  {year} {1966})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Langer}(1968)}]{langernuc}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~S.}\ \bibnamefont
  {Langer}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Theory of
  Nucleation Rates}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {21}},\ \bibinfo
  {pages} {973} (\bibinfo {year} {1968})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Coleman}(1977)}]{coleman1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Sidney}\ \bibnamefont
  {Coleman}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Fate of the
  false vacuum: Semiclassical theory}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {15}},\
  \bibinfo {pages} {2929} (\bibinfo {year} {1977})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Curtis G. Callan Jr.}}\ and\ \citenamefont
  {Coleman}(1977)}]{coleman2}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Curtis G. Callan
  Jr.}}}\ and\ \bibinfo {author} {\bibfnamefont {Sidney}\ \bibnamefont
  {Coleman}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Fate of the
  false vacuum. II. First quantum corrections}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {16}},\ \bibinfo {pages} {1762} (\bibinfo {year} {1977})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Schulman}(1981)}]{schulman}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~S.}\ \bibnamefont
  {Schulman}},\ }\href@noop {} {\emph {\bibinfo {title} {Techniques and
  Applications of Path Integration}}}\ (\bibinfo  {publisher} {Wiley and
  Sons},\ \bibinfo {address} {New York},\ \bibinfo {year} {1981})\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Bulgac}\ \emph {et~al.}(2011)\citenamefont {Bulgac},
  \citenamefont {Luo}, \citenamefont {Magierski}, \citenamefont {Roche},\ and\
  \citenamefont {Yu}}]{Bulgac:2011ee}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Aurel}\ \bibnamefont
  {Bulgac}}, \bibinfo {author} {\bibfnamefont {Yuan-Lung}\ \bibnamefont {Luo}},
  \bibinfo {author} {\bibfnamefont {Piotr}\ \bibnamefont {Magierski}}, \bibinfo
  {author} {\bibfnamefont {Kenneth~J}\ \bibnamefont {Roche}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Yongle}\ \bibnamefont {Yu}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Real-Time Dynamics of Quantized Vortices in a
  Unitary Fermi Superfluid}},}\ }\href {\doibase 10.1126/science.1201968}
  {\bibfield  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo
  {volume} {332}},\ \bibinfo {pages} {1288--1291} (\bibinfo {year}
  {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yefsah}\ \emph {et~al.}(2013)\citenamefont {Yefsah},
  \citenamefont {Sommer}, \citenamefont {Ku}, \citenamefont {Cheuk},
  \citenamefont {Ji}, \citenamefont {Bakr},\ and\ \citenamefont
  {Zwierlein}}]{Yefsah:2013bl}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Tarik}\ \bibnamefont
  {Yefsah}}, \bibinfo {author} {\bibfnamefont {Ariel~T}\ \bibnamefont
  {Sommer}}, \bibinfo {author} {\bibfnamefont {Mark J~H}\ \bibnamefont {Ku}},
  \bibinfo {author} {\bibfnamefont {Lawrence~W}\ \bibnamefont {Cheuk}},
  \bibinfo {author} {\bibfnamefont {Wenjie}\ \bibnamefont {Ji}}, \bibinfo
  {author} {\bibfnamefont {Waseem~S}\ \bibnamefont {Bakr}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Martin~W}\ \bibnamefont {Zwierlein}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Heavy solitons in a fermionic
  superfluid}},}\ }\href {\doibase 10.1038/nature12338} {\bibfield  {journal}
  {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {499}},\ \bibinfo
  {pages} {426--430} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ku}\ \emph {et~al.}(2014)\citenamefont {Ku},
  \citenamefont {Ji}, \citenamefont {Mukherjee}, \citenamefont
  {Guardado-Sanchez}, \citenamefont {Cheuk}, \citenamefont {Yefsah},\ and\
  \citenamefont {Zwierlein}}]{Ku:2014ip}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Mark J~H}\
  \bibnamefont {Ku}}, \bibinfo {author} {\bibfnamefont {Wenjie}\ \bibnamefont
  {Ji}}, \bibinfo {author} {\bibfnamefont {Biswaroop}\ \bibnamefont
  {Mukherjee}}, \bibinfo {author} {\bibfnamefont {Elmer}\ \bibnamefont
  {Guardado-Sanchez}}, \bibinfo {author} {\bibfnamefont {Lawrence~W}\
  \bibnamefont {Cheuk}}, \bibinfo {author} {\bibfnamefont {Tarik}\ \bibnamefont
  {Yefsah}}, \ and\ \bibinfo {author} {\bibfnamefont {Martin~W}\ \bibnamefont
  {Zwierlein}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Motion of a
  Solitonic Vortex in the BEC-BCS Crossover}},}\ }\href {\doibase
  10.1103/PhysRevLett.113.065301} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {113}},\ \bibinfo {pages}
  {065301} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Donadello}\ \emph {et~al.}(2014)\citenamefont
  {Donadello}, \citenamefont {Serafini}, \citenamefont {Tylutki}, \citenamefont
  {Pitaevskii}, \citenamefont {Dalfovo}, \citenamefont {Lamporesi},\ and\
  \citenamefont {Ferrari}}]{Donadello:2014cz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Simone}\ \bibnamefont
  {Donadello}}, \bibinfo {author} {\bibfnamefont {Simone}\ \bibnamefont
  {Serafini}}, \bibinfo {author} {\bibfnamefont {Marek}\ \bibnamefont
  {Tylutki}}, \bibinfo {author} {\bibfnamefont {Lev~P}\ \bibnamefont
  {Pitaevskii}}, \bibinfo {author} {\bibfnamefont {Franco}\ \bibnamefont
  {Dalfovo}}, \bibinfo {author} {\bibfnamefont {Giacomo}\ \bibnamefont
  {Lamporesi}}, \ and\ \bibinfo {author} {\bibfnamefont {Gabriele}\
  \bibnamefont {Ferrari}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Observation of Solitonic Vortices in Bose-Einstein Condensates}},}\ }\href
  {\doibase 10.1103/PhysRevLett.113.065302} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {113}},\ \bibinfo
  {pages} {065302} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Serafini}\ \emph {et~al.}(2015)\citenamefont
  {Serafini}, \citenamefont {Barbiero}, \citenamefont {Debortoli},
  \citenamefont {Donadello}, \citenamefont {Larcher}, \citenamefont {Dalfovo},
  \citenamefont {Lamporesi},\ and\ \citenamefont {Ferrari}}]{Serafini:2015fk}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S}~\bibnamefont
  {Serafini}}, \bibinfo {author} {\bibfnamefont {M}~\bibnamefont {Barbiero}},
  \bibinfo {author} {\bibfnamefont {M}~\bibnamefont {Debortoli}}, \bibinfo
  {author} {\bibfnamefont {S}~\bibnamefont {Donadello}}, \bibinfo {author}
  {\bibfnamefont {F}~\bibnamefont {Larcher}}, \bibinfo {author} {\bibfnamefont
  {F}~\bibnamefont {Dalfovo}}, \bibinfo {author} {\bibfnamefont
  {G}~\bibnamefont {Lamporesi}}, \ and\ \bibinfo {author} {\bibfnamefont
  {G}~\bibnamefont {Ferrari}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Dynamics and Interaction of Vortex Lines in an Elongated Bose-Einstein
  Condensate}},}\ }\href {\doibase 10.1103/PhysRevLett.115.170402} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {115}},\ \bibinfo {pages} {170402} (\bibinfo {year}
  {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ku}\ \emph {et~al.}(2016)\citenamefont {Ku},
  \citenamefont {Mukherjee}, \citenamefont {Yefsah},\ and\ \citenamefont
  {Zwierlein}}]{Ku:2016fk}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Mark J.~H.}\
  \bibnamefont {Ku}}, \bibinfo {author} {\bibfnamefont {Biswaroop}\
  \bibnamefont {Mukherjee}}, \bibinfo {author} {\bibfnamefont {Tarik}\
  \bibnamefont {Yefsah}}, \ and\ \bibinfo {author} {\bibfnamefont {Martin~W.}\
  \bibnamefont {Zwierlein}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Cascade of Solitonic Excitations in a Superfluid Fermi gas: From Planar
  Solitons to Vortex Rings and Lines}},}\ }\href {\doibase
  10.1103/PhysRevLett.116.045304} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {116}},\ \bibinfo {pages}
  {045304} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Prokof'ev}\ \emph {et~al.}(2004)\citenamefont
  {Prokof'ev}, \citenamefont {Ruebenacker},\ and\ \citenamefont
  {Svistunov}}]{Prokofev:2004js}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Nikolay}\ \bibnamefont
  {Prokof'ev}}, \bibinfo {author} {\bibfnamefont {Oliver}\ \bibnamefont
  {Ruebenacker}}, \ and\ \bibinfo {author} {\bibfnamefont {Boris}\ \bibnamefont
  {Svistunov}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Weakly
  interacting Bose gas in the vicinity of the normal-fluid-superfluid
  transition}},}\ }\href {\doibase 10.1103/PhysRevA.69.053625} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume}
  {69}},\ \bibinfo {pages} {053625} (\bibinfo {year} {2004})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Singasaas}\ and\ \citenamefont
  {Ahlers}(1984)}]{SiAh84}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Alan}\ \bibnamefont
  {Singasaas}}\ and\ \bibinfo {author} {\bibfnamefont {Guenter}\ \bibnamefont
  {Ahlers}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Universality of
  static properties near the superfluid transition in He4}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {30}},\ \bibinfo {pages} {5103} (\bibinfo {year}
  {1984})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Crescimanno}\ \emph {et~al.}(2000)\citenamefont
  {Crescimanno}, \citenamefont {Koay}, \citenamefont {Peterson},\ and\
  \citenamefont {Walsworth}}]{crescimanno}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Crescimanno}}, \bibinfo {author} {\bibfnamefont {C.~G.}\ \bibnamefont
  {Koay}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Peterson}}, \
  and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Walsworth}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {{Analytical estimate of the
  critical velocity for vortex pair creation in trapped Bose condensates}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. A}\
  }\textbf {\bibinfo {volume} {62}},\ \bibinfo {pages} {063612} (\bibinfo
  {year} {2000})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Langer}\ and\ \citenamefont {Ambegaokar}(1967)}]{LA}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Langer}}\ and\ \bibinfo {author} {\bibfnamefont {Vinay}\ \bibnamefont
  {Ambegaokar}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Intrinsic
  Resistive Transition in Narrow Superconducting Channels}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev.}\ }\textbf {\bibinfo
  {volume} {164}},\ \bibinfo {pages} {498} (\bibinfo {year}
  {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McCumber}\ and\ \citenamefont {Halperin}(1970)}]{MH}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {McCumber}}\ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Halperin}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Time Scale of
  Intrinsic Resistive Fluctuations in Thin Superconducting Wires}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\
  }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages} {1054} (\bibinfo {year}
  {1970})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Khlebnikov}(2004)}]{Khlebnikov:2004ia}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Khlebnikov}},\ }\bibfield  {title} {{\selectlanguage {English}\enquote
  {\bibinfo {title} {{Quasiparticle Scattering by Quantum Phase Slips in
  One-Dimensional Superfluids}},}\ }}\href {\doibase
  10.1103/PhysRevLett.93.090403} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {93}},\ \bibinfo {pages}
  {090403} (\bibinfo {year} {2004})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Danshita}(2013)}]{Danshita:2013di}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Ippei}\ \bibnamefont
  {Danshita}},\ }\bibfield  {title} {{\selectlanguage {English}\enquote
  {\bibinfo {title} {{Universal Damping Behavior of Dipole Oscillations of
  One-Dimensional Ultracold Gases Induced by Quantum Phase Slips}},}\ }}\href
  {\doibase 10.1103/PhysRevLett.111.025303} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {111}},\ \bibinfo
  {pages} {025303} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\end{thebibliography}%


==> supp_refs.tex <==
\begin{thebibliography}{19}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Morse}\ and\ \citenamefont
  {Feshbach}(1953)}]{SImorsefeshbach}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.M.C.}\ \bibnamefont
  {Morse}}\ and\ \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Feshbach}},\ }\href@noop {} {\emph {\bibinfo {title} {Methods of Theoretical
  Physics}}},\ Vol.~\bibinfo {volume} {2}\ (\bibinfo  {publisher}
  {McGraw-Hill},\ \bibinfo {year} {1953})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Blount}\ and\ \citenamefont {Varma}(1976)}]{SIblount}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E}~\bibnamefont
  {Blount}}\ and\ \bibinfo {author} {\bibfnamefont {C}~\bibnamefont {Varma}},\
  }\bibfield  {title} {\enquote {\bibinfo {title} {{Hydrodynamics of vortex
  generation in flowing superfluid helium}},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {14}},\ \bibinfo {pages} {2888} (\bibinfo {year} {1976})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Schwarz}(1993)}]{SIschwarz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K~W}\ \bibnamefont
  {Schwarz}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Phase slip and
  phase-slip cascades in He4superflow through a small orifice}},}\ }\href@noop
  {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {71}},\ \bibinfo {pages} {259} (\bibinfo {year}
  {1993})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Josephson}(1966)}]{SIjosephson}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.~D.}\ \bibnamefont
  {Josephson}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Relation
  between the superfluid density and order parameter for superfluid He near
  Tc}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Lett.}\ }\textbf {\bibinfo {volume} {21}},\ \bibinfo {pages} {608} (\bibinfo
  {year} {1966})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Donnelly}\ and\ \citenamefont
  {Barenghi}(1998)}]{SIDonnelly:1998ge}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R~J}\ \bibnamefont
  {Donnelly}}\ and\ \bibinfo {author} {\bibfnamefont {C~F}\ \bibnamefont
  {Barenghi}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{The observed
  properties of liquid helium at the saturated vapor pressure}},}\ }\href@noop
  {} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. Chem.}\ }\textbf
  {\bibinfo {volume} {27}},\ \bibinfo {pages} {1217} (\bibinfo {year}
  {1998})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Prokof'ev}\ \emph {et~al.}(2004)\citenamefont
  {Prokof'ev}, \citenamefont {Ruebenacker},\ and\ \citenamefont
  {Svistunov}}]{SIProkofev:2004js}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Nikolay}\ \bibnamefont
  {Prokof'ev}}, \bibinfo {author} {\bibfnamefont {Oliver}\ \bibnamefont
  {Ruebenacker}}, \ and\ \bibinfo {author} {\bibfnamefont {Boris}\ \bibnamefont
  {Svistunov}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Weakly
  interacting Bose gas in the vicinity of the normal-fluid-superfluid
  transition}},}\ }\href {\doibase 10.1103/PhysRevA.69.053625} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume}
  {69}},\ \bibinfo {pages} {053625} (\bibinfo {year} {2004})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Varoquaux}(2015)}]{SIvaroquauxrmp}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Eric}\ \bibnamefont
  {Varoquaux}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Anderson{\textquoteright}s considerations on the flow of superfluid helium:
  Some offshoots}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {87}},\ \bibinfo {pages} {803}
  (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Harrison}\ and\ \citenamefont
  {Mendelssohn}(1974)}]{SIharrison}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~J.}\ \bibnamefont
  {Harrison}}\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Mendelssohn}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Superfluid
  4He Velocities in Narrow Channels between 1.8 and 0.3 K}},}\ }in\ \href@noop
  {} {\emph {\bibinfo {booktitle} {Low Temperature Physics}}},\ \bibinfo
  {editor} {edited by\ \bibinfo {editor} {\bibfnamefont {T~D}\ \bibnamefont
  {Timmerhaus}}}\ (\bibinfo  {publisher} {Springer},\ \bibinfo {address} {New
  York},\ \bibinfo {year} {1974})\ p.\ \bibinfo {pages} {298}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Duc}\ \emph {et~al.}(2015)\citenamefont {Duc},
  \citenamefont {Savard}, \citenamefont {Petrescu}, \citenamefont {Rosenow},
  \citenamefont {Del~Maestro},\ and\ \citenamefont {Gervais}}]{SIduc}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Pierre-Francois}\
  \bibnamefont {Duc}}, \bibinfo {author} {\bibfnamefont {Michel}\ \bibnamefont
  {Savard}}, \bibinfo {author} {\bibfnamefont {Matei}\ \bibnamefont
  {Petrescu}}, \bibinfo {author} {\bibfnamefont {Bernd}\ \bibnamefont
  {Rosenow}}, \bibinfo {author} {\bibfnamefont {Adrian}\ \bibnamefont
  {Del~Maestro}}, \ and\ \bibinfo {author} {\bibfnamefont {Guillaume}\
  \bibnamefont {Gervais}},\ }\bibfield  {title} {\enquote {\bibinfo {title}
  {{Critical flow and dissipation in a quasi-one-dimensional superfluid}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Science Adv.}\
  }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages} {e1400222} (\bibinfo
  {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Neely}\ \emph {et~al.}(2010)\citenamefont {Neely},
  \citenamefont {Samson}, \citenamefont {Bradley}, \citenamefont {Davis},\ and\
  \citenamefont {Anderson}}]{SIneely}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.~W.}\ \bibnamefont
  {Neely}}, \bibinfo {author} {\bibfnamefont {E.~C.}\ \bibnamefont {Samson}},
  \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont {Bradley}}, \bibinfo
  {author} {\bibfnamefont {M.~J.}\ \bibnamefont {Davis}}, \ and\ \bibinfo
  {author} {\bibfnamefont {B.~P.}\ \bibnamefont {Anderson}},\ }\bibfield
  {title} {\enquote {\bibinfo {title} {{Observation of Vortex Dipoles in an
  Oblate Bose-Einstein Condensate}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {104}},\
  \bibinfo {pages} {160401} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ramanathan}\ \emph {et~al.}(2011)\citenamefont
  {Ramanathan}, \citenamefont {Wright}, \citenamefont {Muniz}, \citenamefont
  {Zelan}, \citenamefont {Hill}, \citenamefont {Lobb}, \citenamefont
  {Helmerson}, \citenamefont {Phillips},\ and\ \citenamefont
  {Campbell}}]{SIramanathan}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Ramanathan}}, \bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont
  {Wright}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Muniz}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Zelan}}, \bibinfo
  {author} {\bibfnamefont {W.~T.}\ \bibnamefont {Hill}}, \bibinfo {author}
  {\bibfnamefont {C.~J.}\ \bibnamefont {Lobb}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Helmerson}}, \bibinfo {author}
  {\bibfnamefont {W.~D.}\ \bibnamefont {Phillips}}, \ and\ \bibinfo {author}
  {\bibfnamefont {G.~K.}\ \bibnamefont {Campbell}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Superflow in a Toroidal Bose-Einstein
  Condensate: An Atom Circuit with a Tunable Weak Link}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {106}},\ \bibinfo {pages} {130401} (\bibinfo {year}
  {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Raman}\ \emph {et~al.}(1999)\citenamefont {Raman},
  \citenamefont {K{\"o}hl}, \citenamefont {Onofrio}, \citenamefont {Durfee},
  \citenamefont {Kuklewicz}, \citenamefont {Hadzibabic},\ and\ \citenamefont
  {Ketterle}}]{SIraman}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Raman}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {K{\"o}hl}},
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Onofrio}}, \bibinfo
  {author} {\bibfnamefont {D.~S.}\ \bibnamefont {Durfee}}, \bibinfo {author}
  {\bibfnamefont {C.~E.}\ \bibnamefont {Kuklewicz}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Hadzibabic}}, \ and\ \bibinfo {author}
  {\bibfnamefont {W.}~\bibnamefont {Ketterle}},\ }\bibfield  {title} {\enquote
  {\bibinfo {title} {{Evidence for a Critical Velocity in a Bose-Einstein
  Condensed Gas}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {83}},\ \bibinfo {pages}
  {2502} (\bibinfo {year} {1999})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Weimer}\ \emph {et~al.}(2015)\citenamefont {Weimer},
  \citenamefont {Morgener}, \citenamefont {Singh}, \citenamefont {Siegl},
  \citenamefont {Hueck}, \citenamefont {Luick}, \citenamefont {Mathey},\ and\
  \citenamefont {Moritz}}]{SIweimer}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Wolf}\ \bibnamefont
  {Weimer}}, \bibinfo {author} {\bibfnamefont {Kai}\ \bibnamefont {Morgener}},
  \bibinfo {author} {\bibfnamefont {Vijay~Pal}\ \bibnamefont {Singh}}, \bibinfo
  {author} {\bibfnamefont {Jonas}\ \bibnamefont {Siegl}}, \bibinfo {author}
  {\bibfnamefont {Klaus}\ \bibnamefont {Hueck}}, \bibinfo {author}
  {\bibfnamefont {Niclas}\ \bibnamefont {Luick}}, \bibinfo {author}
  {\bibfnamefont {Ludwig}\ \bibnamefont {Mathey}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Henning}\ \bibnamefont {Moritz}},\ }\bibfield  {title}
  {\enquote {\bibinfo {title} {{Critical Velocity in the BEC-BCS Crossover}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\
  }\textbf {\bibinfo {volume} {114}},\ \bibinfo {pages} {095301} (\bibinfo
  {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chien}\ \emph {et~al.}(2015)\citenamefont {Chien},
  \citenamefont {Peotta},\ and\ \citenamefont {Di~Ventra}}]{SIchien}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Chih-Chun}\
  \bibnamefont {Chien}}, \bibinfo {author} {\bibfnamefont {Sebastiano}\
  \bibnamefont {Peotta}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Massimiliano}\ \bibnamefont {Di~Ventra}},\ }\bibfield  {title} {\enquote
  {\bibinfo {title} {{Quantum transport in ultracold atoms}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature Phys.}\ }\textbf {\bibinfo
  {volume} {11}},\ \bibinfo {pages} {998} (\bibinfo {year} {2015})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Capogrosso-Sansone}\ \emph
  {et~al.}(2010)\citenamefont {Capogrosso-Sansone}, \citenamefont {Giorgini},
  \citenamefont {Pilati}, \citenamefont {Pollet}, \citenamefont {Prokof'ev},
  \citenamefont {Svistunov},\ and\ \citenamefont
  {Troyer}}]{SICapogrossoSansone:2010kt}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B}~\bibnamefont
  {Capogrosso-Sansone}}, \bibinfo {author} {\bibfnamefont {S}~\bibnamefont
  {Giorgini}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Pilati}},
  \bibinfo {author} {\bibfnamefont {L}~\bibnamefont {Pollet}}, \bibinfo
  {author} {\bibfnamefont {N}~\bibnamefont {Prokof'ev}}, \bibinfo {author}
  {\bibfnamefont {B}~\bibnamefont {Svistunov}}, \ and\ \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Troyer}},\ }\bibfield  {title} {\enquote
  {\bibinfo {title} {{The Beliaev technique for a weakly interacting Bose
  gas}},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {New J.
  Phys.}\ }\textbf {\bibinfo {volume} {12}},\ \bibinfo {pages} {043010}
  (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Langer}\ and\ \citenamefont {Fisher}(1967)}]{SIlanger}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Langer}}\ and\ \bibinfo {author} {\bibfnamefont {Michael}\ \bibnamefont
  {Fisher}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Intrinsic
  Critical Velocity of a Superfluid}},}\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {19}},\
  \bibinfo {pages} {560} (\bibinfo {year} {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Singasaas}\ and\ \citenamefont
  {Ahlers}(1984)}]{SISiAh84}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Alan}\ \bibnamefont
  {Singasaas}}\ and\ \bibinfo {author} {\bibfnamefont {Guenter}\ \bibnamefont
  {Ahlers}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Universality of
  static properties near the superfluid transition in He4}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {30}},\ \bibinfo {pages} {5103} (\bibinfo {year}
  {1984})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Langer}\ and\ \citenamefont {Ambegaokar}(1967)}]{SILA}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Langer}}\ and\ \bibinfo {author} {\bibfnamefont {Vinay}\ \bibnamefont
  {Ambegaokar}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Intrinsic
  Resistive Transition in Narrow Superconducting Channels}},}\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev.}\ }\textbf {\bibinfo
  {volume} {164}},\ \bibinfo {pages} {498} (\bibinfo {year}
  {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McCumber}\ and\ \citenamefont {Halperin}(1970)}]{SIMH}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {McCumber}}\ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Halperin}},\ }\bibfield  {title} {\enquote {\bibinfo {title} {{Time Scale of
  Intrinsic Resistive Fluctuations in Thin Superconducting Wires}},}\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\
  }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages} {1054} (\bibinfo {year}
  {1970})}\BibitemShut {NoStop}%
\end{thebibliography}%

